MARIO: Model Agnostic Recipe for Improving OOD Generalization of Graph Contrastive Learning

In this work, we investigate the problem of out-of-distribution (OOD) generalization for unsupervised learning methods on graph data. This scenario is particularly challenging because graph neural networks (GNNs) have been shown to be sensitive to distributional shifts, even when labels are available. To address this challenge, we propose a \underline{M}odel-\underline{A}gnostic \underline{R}ecipe for \underline{I}mproving \underline{O}OD generalizability of unsupervised graph contrastive learning methods, which we refer to as MARIO. MARIO introduces two principles aimed at developing distributional-shift-robust graph contrastive methods to overcome the limitations of existing frameworks: (i) Information Bottleneck (IB) principle for achieving generalizable representations and (ii) Invariant principle that incorporates adversarial data augmentation to obtain invariant representations. To the best of our knowledge, this is the first work that investigates the OOD generalization problem of graph contrastive learning, with a specific focus on node-level tasks. Through extensive experiments, we demonstrate that our method achieves state-of-the-art performance on the OOD test set, while maintaining comparable performance on the in-distribution test set when compared to existing approaches. The source code for our method can be found at: https://github.com/ZhuYun97/MARIO

==> sections/preliminary.tex <==
\section{Preliminaries~\label{sec:pre}}

\subsection{Notations}
\noindent Let $\mathcal{G},\mathcal{Y}$ represent input and label space respectively. $f_\phi(\cdot)=p_\omega\circ g_\theta(\cdot)$ represents graph predictor which consists of a GNN encoder $g_\theta(\cdot)$ and a classifier $p_\omega(\cdot)$. The graph predictor $f_\phi: \mathcal{G}\rightarrow\mathcal{Y}$ maps instance $G=(A,X) \in \mathcal{G}$ to label $Y \in \mathcal{Y}$ where $A \in \mathbb{R}^{N \times N}$ is the adjacent matrix and $X \in \mathbb{R}^{N \times D}$ is the node attribute matrix. Here, $N$, $D$ denote the number of nodes and attributes, respectively. To measure the discrepancy between the prediction and the ground-truth label, a loss function $\ell_{\text{sup}}$ is used (\eg, cross-entropy loss, mean square error). For unsupervised learning, a pretext loss $\ell_{\text{unsup}}$ is applied (\eg, InfoNCE loss~\cite{cpc}).
\subsection{Problem Statement}
\textbf{Graph OOD Generalization:} Given training set $\mathcal{G}^{\text{train}}={(G_i,Y_i)}_{i=1}^N$ containing $N$ instances that are drawn from training distribution $P_{\text{train}}(G,Y)$. In the supervised setting, it aims to learn an optimal graph predictor $f^*$ that can exhibit the best generalization performance on the data sampled from the test distribution:
% It has to note that in OOD scenario $P_{\text {test }}(\mathcal{G}, Y) \neq P_{\text {train }}(\mathcal{G}, Y)$ which is different to IID assumption:
\begin{equation}
f_\phi^*=\arg \min _{f_\phi} \mathbb{E}_{G, Y \sim P_{\text {test }}}\left[\ell_{\text{sup}}\left(f_\phi(G), Y\right)\right],
\end{equation}
where $P_{\text {test }}(G, Y) \neq P_{\text {train }}(G, Y)$ means there exists a distribution shift between training and testing sets. Such a shift may lead to the optimal predictor trained on the training set (\ie, minimizing $\mathbb{E}_{G, Y \sim P_{\text {train }}}\left[\ell_{\text{sup}}\left(f_\phi(G), Y\right)\right]$) can not generalize on the testing set.
% \paragraph{Unsupervised graph OOD generalization} Given an unlabelled training data set $\mathcal{G}^{train}=\{(G_i)\}_{i=1}^N$ containing N instances from training distribution $P_{\text{train}}(\mathcal{G})$. In the unsupervised setting, to learn an optimal graph encoder $g^*$ that performs well on the pretext task, for instance, $\mathbb{E}_{\mathcal{G}, Y \sim P_{\text {train }}}\left[\ell_{\text{unsup}}\left(g_\theta(\mathcal{G}), g(\mathcal{G}^-), g(\mathcal{G}^+)\right)\right]$ where $\mathcal{G},\mathcal{G}^+$ are sampled from joint distribution and $\mathcal{G},\mathcal{G}^-$ are sampled from the product of marginal distributions. In order to evaluate the pre-trained model, it is common to use linear evaluation which we fix the pre-trained model and additionally train a linear classifier $p$ with labeled data set $D~P_{\text {train }}(\mathcal{G}, Y)$. And lastly, we test the graph predictor  $p\circ g$ on the test data set $P_{\text {test }}(\mathcal{G}, Y)$, where $P_{\text {test }}(\mathcal{G}, Y) \neq P_{\text {train }}(\mathcal{G}, Y)$. 
%\footnote{For notation uncluttered, we assume only one graph in the training set which is commonly found in the node classification task.}

\noindent\textbf{Self-Supervised Graph Learning:} 
The most representative self-supervised graph learning method is graph contrastive learning (GCL) recently~\cite{rosa,grace,graphcl,costa,bgrl,dgi,mvgrl}. In this subsection, we focus on introducing the main components and formulations used in GCL. GCL hopes to learn a generic feature extractor without human annotations through a pre-defined pre-text task (\eg, instance discrimination). Most of them~\cite{rosa,grace,graphcl,costa,bgrl,dgi,mvgrl} consist of three main components: (1) view generation, (2) view encoding and (3) representation contrasting. The pipeline is depicted in Figure~\ref{fig:contrast}. Firstly, given an input graph $G$, in the phase of view generation, two graph augmentation $\tau_{\alpha}(\cdot|G),\tau_{\beta}(\cdot|G)\sim\mathcal{T}$\footnote{$\mathcal{T}$ is an augmentation pool which can consist of various augmentation techniques like edge dropping, attribute masking, subgraph and etc~\cite{graphcl}.} will be applied on the original graph to generate the augmented views $G_\alpha, G_\beta$. Secondly, these augmented graphs will be fed into GNN-based encoding models~\cite{gcn,gat,gin,sage} to obtain node representations $U, V \in \mathbb{R}^{N \times D}$.
% We use $u,v \in \mathbb{R}^{1 \times D}$ to represent the random variables of node representation. 
Lastly, an unsupervised loss function will be applied to these representations. Taking the commonly used InfoNCE loss~\cite{cpc} as an example:
\begin{equation}
\begin{aligned}
\mathcal{L} _ {MI} & \left(U, V\right)=-\mathbb{E}_{u,v \sim P_{U,V}}\left[\operatorname{sim}\left(u, v\right)\right] \\
+ & \mathbb{E}_{u \sim P_U} \log \mathbb{E}_{v^- \sim P_V} \left[  e^{\operatorname{sim}\left(u, v^-\right)}\right],
\end{aligned}
\label{equ:con}
\end{equation}
where $\operatorname{sim}(u,v)$ is a score function (\eg,  cosine similarity), $u, v=g_{\theta}(G_{\alpha}),g_{\theta}(G_{\beta})$. More specifically, it can be formulated:
\begin{equation}
\begin{aligned}
\mathcal{L} _ {MI} & \left(g_\theta;\mathcal{G},\pi\right)=-\underset{G \in \mathcal{G}}{\mathbb{E}} \mathbb{E} _{\tau_\alpha, \tau_\beta \in \mathcal{T}}\left\|g_\theta(\tau_\alpha(G))-g_\theta\left(\tau_\beta(G)\right)\right\|^2 \\
+ & \underset{G \in \mathcal{G}}{\mathbb{E}} \log \underset{G^{\prime} \in \mathcal{G}}{\mathbb{E}}\mathbb{E}_{\tau^{\prime} \in \mathcal{T}}\left[  e^{\left\|g_\theta\left(\tau_\alpha\left(G\right)\right)-g_\theta\left(\tau^{\prime}(G^\prime)\right)\right\|^2}\right]
\end{aligned}
\label{equ:con}
\end{equation}
For simplicity, we assume that $\|g_\theta(G)\|=1$ for every $G \in \mathcal{G}$. By minimizing this loss, the former term (aka alignment loss $\mathcal{L}_{\text{align}}$~\cite{wang2020understanding}) pulls positive pairs ($u,v \sim P_{U,V}$) together by encouraging their similarity, and the latter term (aka uniformity loss $\mathcal{L}_{\text{uniform}}$~\cite{wang2020understanding}) pushes negative pairs ($u,v^- \sim P_U \otimes P_V$) apart. In order to evaluate the pre-trained model, an additional trainable linear classifier (\ie, one-layer MLP) will be built on top of the frozen encoder:

\begin{equation}
p_\omega^*=\arg \min _{p_\omega} \mathbb{E}_{G, Y \sim P_{\text {train }}}\left[\ell_{\text{sup}}\left(p_\omega \circ g_\theta^*(G), Y\right)\right],
\end{equation}
where $g_\theta^*(\cdot)$ is obtained by minimizing Equation~\ref{equ:con} without labels. For evaluating pre-trained model, the optimal graph predictor $f_\phi^* =  p_\omega^* \circ g_\theta^*$ will be applied to testing data. In the previous works, they assume training data and testing data are sampled from an identical distribution. So some spurious patterns extracted by pre-trained models can benefit downstream dataset.

\zy{\noindent\textbf{Self-Supervised OOD Generalization on Graphs:}}
% The design of most existing GCL methods does not consider the OOD scenario. In other words, few works explore the self-supervised OOD generalization on graphs. For achieving this aim, we hope to learn a feature extractor $g_\theta^\star$ that can dig invariant patterns rather than spurious features (\eg, variant features with environments) which is more strict than in the last subsection. So, we need to modify the main components in current GCL methods which will be discussed in Section~\ref{sec:method}.
Existing GCL methods generally lack consideration of the OOD scenario. In other words, few works have specifically explored self-supervised OOD generalization on graphs. To address this limitation, our goal is to learn a feature extractor $g_\theta^\star$ that can effectively capture invariant rationales while avoiding spurious features, such as those influenced by varying environments, aiming for downstream node classification task. 
% For instance, taking the molecule property prediction as downstream task, we hope the encoder can recognize the functional group which will decide the property of molecule.  
We assume $\Phi(G)$ is invariant rationales of input instance $G$ which is stable in different environments (augmentations) following invariance assumption~\cite{ood-survey,good-survey}. We hope the pre-trained model can achieve this objective\footnote{We assume the augmentation function will not change the semantic labels of the original input here.}:
\begin{equation}
    g_\theta^{\star}(G_e)=g_\theta^{\star}(G_{e^\prime}) = \Phi(G),  \quad \forall e,e^\prime \in \operatorname{supp}\left(\mathcal{E}_{t r}\right)
\label{equ:goal}
\end{equation}
where $\mathcal{E}_{t r}$ denotes the set of training environments and $\mathbb{E}\left[Y \mid \Phi\left(G_e\right)\right]=\mathbb{E}\left[Y \mid \Phi\left(G_{e^{\prime}}\right)\right]$ which means invariant rationales exhibiting the stable correlation with semantic labels across different environments. However, during pre-training, we have no access to labels under self-supervised setting. Here, we build a connection between pre-text loss $\mathcal{L}_{M I}\left(g_\theta ; \mathcal{G}, \pi\right)$ and downstream loss $\mathcal{R}\left(g_\theta ; \mathcal{G}^{\operatorname{tar}}\right)$~\cite{arcl,huang2023towards}:
\begin{equation}
\begin{aligned}
\mathcal{R}\left(p_\omega \circ g_\theta ; \mathcal{G}_\pi\right) \leq 
& c\|p_\omega\| \sqrt{K \sigma}\left(\mathcal{L}_{\text {align }}(g_\theta ; \mathcal{G}, \pi)\right)^{\frac{1}{4}} \\ 
& +\|p_\omega\| \zeta (\sigma, \delta) \\
& +\sum_{k=1}^K \mathcal{G}_\pi\left(C_k\right)\left\|e_k-p_\omega \circ \mu_k\left(g_\theta ; \mathcal{G}_\pi\right)\right\|
\end{aligned}
\label{equ:cl_down}
\end{equation}
where $c$ is an absolute constant, $\zeta (\sigma, \delta)$ is of a constant which only depends on $(\sigma, \delta)$-augmentation~\cite{huang2023towards}, $C_k \subseteq \mathcal{G}$ is the set of all points in class $k$, $\mu_k(g_\theta ; \mathcal{G}):=\mathbb{E}_{G \sim \mathcal{G}} g_\theta(G) \text { for } k \in[K]$, $\pi$ is a certain distribution for augmentation $\tau \sim \mathcal{T}(\pi)$, the complete deduction and more illustrations can be found in Appendix. 
% The first term in Equation~\ref{equ:cl_down} is the alignment loss which is optimized during pre-training on $\mathcal{G}$. The second term is determined solely by $(\sigma,\delta)$ quantity of the data augmentation. Larger $\sigma$ and smaller $\delta$ induce smaller $\zeta(\sigma,\delta)$. The third term is related to the linear layer $p$ on top of $g$, and will be minimized in downstream training, where each class center is converted to the corresponding ground-truth label. If the regularization term $L_{reg}$ is appropriately chosen, the class centers can be distinguished from each other, and the third term can be reduced to 0 by $h$.
The first term of Equation~\ref{equ:cl_down} is the alignment loss optimized during pre-training on $\mathcal{G}$. 
The second term is determined by the $(\sigma,\delta)$ quantity of the data augmentation, with larger $\sigma$ and smaller $\delta$ resulting in smaller $\zeta(\sigma,\delta)$.
The third term is associated with the linear layer $p$ and is minimized in downstream training. The class centers can be distinguished by choosing an appropriate regularization term $\mathcal{L}_{\text{uniform}}$, leading to the third term becoming 0 via $h$.
In short, Equation~\ref{equ:cl_down} implies that contrastive learning on distribution $\mathcal{G}$ with augmentation function $\tau \sim \mathcal{T}(\pi)$ essentially optimizes the supervised risk on the augmented distribution $\mathcal{G}_\tau$. So, even without labels, we can approach the goal formulated as Equation~\ref{equ:goal} during pre-training to some extent, through modifying the main components in current GCL methods which will be discussed in Section~\ref{sec:method}.

% The above equation means $g_\theta^{\star}$ can extract invariant rationales across different environments. In order to achieve this, it is necessary to modify the main components in current GCL methods which will be discussed in Section~\ref{sec:method}.

%The linear classifier has risks to learn spurious correlation which may destroy the node embeddings. In order to avoid this, \cite{shi2022robust} adopts partial test data rather than training data for training linear classifier, but it is unfair to compare with supervised methods. So in this work, we still use training data to learn the linear head. 
For evaluating the pre-trained models, the linear evaluation protocol mentioned in the last subsection will be used: 
\begin{equation}
p_\omega^*=\arg \min _{p_\omega} \mathbb{E}_{G, Y \sim P_{\text {train }}}\left[\ell_{\text{sup}}\left(p_\omega \circ g_\theta^\star(G), Y\right)\right],
\end{equation}
where pre-trained model $g_\theta^\star$ is frozen, and the linear classifier $p_\omega$ is trained with training data\footnote{To maintain fairness in the evaluation, we choose to train the linear head using the training data, rather than using partial test data as done in \cite{shi2022robust}. Although the linear classifier has risks of learning spurious correlations that could impact the node embeddings.}. The difference with the last subsection is $P_{\text {test }}(G, Y) \neq P_{\text {train }}(G, Y)$ which means there exist distribution shifts between training and testing data. This implies that the feature extractor must extract more invariant features to mitigate the risk of overfitting on the training data and ensure better generalization performance under distribution shifts.

% This requirement is more stringent compared to the previous subsection. To achieve this, we propose modifications to the main components of current GCL methods, which will be discussed in detail in Section~\ref{sec:method}.
% The design of existing GCL methods does not consider the OOD scenario. In other words, few works explore the self-supervised OOD generalization on graphs. In this subsection, we will simply analyze the drawbacks of current GCL methods while facing OOD scenario based on two main components and build a connection between GCL methods and OOD methods. For the view generation, inspired by invariant learning~\cite{irm,groupdro,arcl}, the alignment loss can be reformulated as:
% \begin{equation}
% \mathcal{L}_{\mathrm{align}^*}(g_{\theta} ; \mathcal{G}):=\underset{G \in \mathcal{G}}{\mathbb{E}} \sup _{\tau, \tau^{\prime} \in \mathcal{T}}\left\|g_{\theta}(\tau(G))-g_{\theta}\left(\tau^{\prime}(G)\right)\right\|^2,
% \end{equation}
% which replaces the expectation operator in Equation~\ref{equ:con} with supremum operator. This objective is a uniform version of original alignment loss which can make the representation varies less under different augmentation functions and result in more invariant features. In order to achieve this goal, we can adjust the view generation to approximately approach the supremum operator which will be further discussed in Section~\ref{sec:aug}. 

% Regarding the representation contrasting component, the original contrastive loss aims to maximize the lower bound of mutual information between positive pairs which will contain redundant information. Motivated by Information Bottleneck~\cite{dib,gib}, we reformulate Equation~\ref{equ:con} as Equation~\ref{equ:cmi_tmp} which hopes to exclude redundant information and find minimal sufficient representation\footnote{For self-supervised methods, their aim is to find a generic feature extractor that is agnostic to downstream tasks. But in this work, we focus on node-level tasks. If given label information, there exists explicit redundant information can be excluded.}:
% \begin{equation}
% \begin{aligned}
%     \mathcal{L}_{\mathrm{rob}}&=\argmax I_{\theta}(U;V) - \gamma \underbrace{I_{\theta}(U;V \mid \hat{Y})}_{\text{Redundant info}}
% \end{aligned}
% \label{equ:cmi_tmp}
% \end{equation}
% where $I_\theta(\cdot)$ represents mutual information estimator, $\gamma > 0$ controls the trade-off between compression and performance, and $\hat{Y}$ denotes label\footnote{For unsupervised setting, it denotes pseudo label or protocols.} information of the downstream task.
% By adopting this learning paradigm, the trained model can effectively mitigate overfitting and exhibit increased resilience against distribution shifts. More illustrations can be found in Section~\ref{sec:cmi}.

% As for evaluation, we also adopt the linear evaluation protocol~\cite{simclr}. Using the frozen pre-trained model to extract node embeddings, and using training data is train an additional linear classifier to evaluate the performance:
% \begin{equation}
% p_\omega^*=\arg \min _{p_\omega} \mathbb{E}_{G, Y \sim P_{\text {train }}}\left[\ell_{\text{sup}}\left(p_\omega \circ g_\theta^\star(G), Y\right)\right],
% \end{equation}
% The difference with the last subsection is $P_{\text {test }}(G, Y) \neq P_{\text {train }}(G, Y)$ which means there exist distribution shifts between training and testing data. This implies that the feature extractor must extract more invariant features to mitigate the risk of overfitting on the training data and ensure better generalization performance under distribution shifts.

% Contrastive learning seems to have better generalization on OOD test data by maximizing the lower bound of mutual information of positive pairs. Specifically, considering the augmented data from different domains, contrastive learning will align positive pairs from different domains, leading to extracting more casual patterns. Take the citation network as an example, where the categorization of scientific publications should not depend on the node degree. By employing augmentation techniques such as edge dropping, if there is a degree shift in the downstream test set, contrastive learning methods can achieve favorable generalization performance. Empirically, \cite{shi2022robust} found contrastive learning methods are more robust to distribution shift compared to supervised method~\cite{erm} in the computer vision domain. In this work, we will investigate how current graph contrastive learning methods perform on the graph OOD test set and provide a model-agnostic recipe for improving OOD generalization of the current contrastive methods which is coined as MARIO.
% By minimizing this loss, we can maximize the mutual information between positive pairs meanwhile maximize the mutual information between the input graph and representations~\cite{}. A detailed illustration can be found in Appendix. 


\begin{figure}
    \centering
    \includegraphics[scale=0.5]{figures/contrastive.eps}
    \caption{The pipeline of graph contrastive learning.}
    \label{fig:contrast}
\end{figure}

==> sections/related.tex <==
\section{Related Works}
\subsection{Self-supervised Graph Learning}
% With the eye-catching success of self-supervised on computer vision domain~\cite{moco,simclr,byol,raft,simsiam,mae}, self-supervised graph learning has been booming recently~\cite{rosa,grace,graphcl,bgrl,dgi,mvgrl,gmae,costa}. Specifically, self-supervised graph learning can be categorized into three main kinds: predictive methods, generative methods, and contrastive methods~\cite{wu2021self}. Predictive methods need to design prediction-based pre-training tasks (\eg, degree prediction~\cite{hu2020strategies}) based on self-generative labels by statistical analysis~\cite{hu2020strategies}. 
% Generative methods focus on learning intra-data information within graphs through feature/edge reconstruction~\cite{gae,gmae}. Recently, the generative-based masked autoencoders (e.g., GraphMAE~\cite{gmae}) show their superior performance across different tasks by reconstructing masked features.
% Contrastive methods focus on learning inter-data information between graphs by drawing positive data pairs closer and pushing away the negative data pairs in the representation space.
\noindent The remarkable success of self-supervised learning in the field of computer vision~\cite{moco,simclr,byol,raft,simsiam,mae}, has sparked a surge of interest in self-supervised graph learning~\cite{rosa,grace,graphcl,bgrl,dgi,mvgrl,gmae,costa}. Self-supervised graph learning can be broadly categorized into three main types: predictive methods, generative methods, and contrastive methods~\cite{wu2021self}.
Predictive methods require the design of prediction-based pre-training tasks, such as degree prediction, which utilize self-generated labels derived from statistical analysis~\cite{hu2020strategies}.
Generative methods aim to learn intra-data information within graphs by focusing on feature or edge reconstruction~\cite{gae,gmae}. Recently, generative-based masked autoencoders like GraphMAE have demonstrated superior performance across various tasks by reconstructing masked features.
Contrastive methods, on the other hand, emphasize learning inter-data information between graphs by bringing positive data pairs closer together and pushing negative data pairs apart in the representation space.

% Both generative and contrastive methods have made significant progress in the graph domain, surpassing supervised methods in certain scenarios even without human annotations~\cite{gmae,grace,rosa,mvgrl}.
% However, most current graph self-supervised learning methods are under the in-distribution (ID) assumption, where the distribution of the training set is assumed to be identical to the test set. In reality, distribution shifts often occur between the training and test sets. While various self-supervised graph learning methods are superior to supervised methods on ID test sets, their performance on out-of-distribution (OOD) test sets compared to supervised methods is still under exploration. This naturally raises the question: Are graph self-supervised learning methods more robust than supervised methods?

Indeed, both generative and contrastive methods have made remarkable strides in the graph domain, surpassing supervised methods in certain scenarios even in the absence of human annotations~\cite{gmae,grace,rosa,mvgrl,zhu2023sgl,zhang2023structure}. However, most current graph self-supervised learning methods operate under the in-distribution (ID) assumption, where the training set's distribution is presumed to be identical to that of the test set. In reality, distribution shifts frequently occur between training and test sets. Although various self-supervised graph learning methods exhibit superior performance compared to supervised methods on ID test sets, their robustness and performance on out-of-distribution (OOD) test sets, in comparison to supervised methods, are still being explored. This naturally raises the question: Are graph self-supervised learning methods inherently more robust than supervised methods?

In this work, we will investigate the robustness of graph self-supervised methods in the face of distribution shifts. And we provide a model-agnostic recipe for improving the OOD generalization of graph contrastive learning methods \zy{which does not rely on the choice of models}. \haizhou{how is it model-agnostic specifically?} By addressing this research question, we provide valuable insights and practical guidelines for improving the performance of unsupervised graph contrastive learning in scenarios with distribution shifts.

\subsection{Out-of-Distribution Generalization on Graphs}
% Out-of-distribution generalization (aka domain generalization) algorithm is designed to achieve satisfactory generalization performance while facing unknown distribution shifts~\cite{ood-survey}. Due to the growing need for handling unseen data in real-world scenarios, this algorithm has gained significant attention within the research community. The combination of graph machine learning and OOD generalization (\ie, OOD generalization on graphs), holds great promise and serves as a valuable research direction for enhancing the deployment of graph machine learning models in real-world applications~\cite{good-survey}. 
\noindent Out-of-distribution generalization (aka domain generalization) algorithm, is specifically developed to achieve satisfactory generalization performance when confronted with unknown distribution shifts~\cite{ood-survey}. Due to the growing need for handling unseen data in real-world scenarios, this algorithm has garnered substantial attention within the research community. \zy{Specifically, robust optimization~\cite{groupdro,hu2018does}, invariant representation/predictor learning~\cite{irm,sparseirm} and causal approaches~\cite{peters2016causal,heinze2018causal} are proposed to deal with such problems.} \haizhou{What is the main idea of these DG algorithms? Briefly introduce it.} The combination of graph machine learning and OOD generalization (\ie, OOD generalization on graphs), presents a promising research direction. It holds the potential to enhance the deployment of graph machine learning models in real-world applications, making them more robust and adaptable to diverse and evolving data distributions~\cite{good-survey}. \zy{It is worth noting that there are related topics such as graph domain adaptation~\cite{wu2020unsupervised} and graph transfer learning~\cite{zhu2021transfer}. The key distinction lies in the fact that these approaches typically assume access to a subset of the test domains for adapting GNN models. In contrast, graph domain generalization does not rely on any samples from the test domains, making it distinct from these aforementioned approaches.}

Recently, some works explore the generalization of graph neural networks on graph OOD data~\cite{eerm,gil,dir,rgcl}, but most works mostly focus on graph-level tasks. It is more challenging to deal with node-level tasks due to the interconnection of the graph structure. EERM \cite{eerm} is the first work to deal with node-level graph OOD problems by generating multiple graphs from environment generators and minimizing the mean and variance of risks from multiple environments to capture invariant features. But this work needs to use label information to extract causal patterns. \haizhou{Only one work?} If labels are unavailable or limited, how to train a model with good generalization without supervision is essential but still under exploration. In the computer vision domain, \cite{shi2022robust} found contrastive learning methods are more robust compared to supervised methods. But it is unknown whether graph self-supervised learning methods are robust to distribution shifts. In this work, we will explore the robustness of graph self-supervised methods under distribution shifts.

In recent research, some studies have started exploring the generalization of graph neural networks on out-of-distribution (OOD) graph data~\cite{eerm,gil,dir,rgcl}. However, most of these works have primarily focused on graph-level tasks, while dealing with node-level tasks poses greater challenges due to the interconnected nature of graph structures.
EERM~\cite{eerm} is the first work to address node-level OOD problems in graphs by generating multiple graphs from environment generators and minimizing the mean and variance of risks across multiple environments to capture invariant features. However, this approach relies on label information to extract causal patterns. When labels are unavailable or limited, training a model with good generalization in the absence of supervision becomes crucial but remains an ongoing exploration.

In the computer vision domain, a recent study~\cite{shi2022robust} found that contrastive learning methods exhibit greater robustness compared to supervised methods. However, it remains unknown whether graph self-supervised learning methods possess similar robustness to distribution shifts. \zy{It is worth noting that distribution shifts in graph data tend to be more intricate, with data points (nodes) interconnected through the graph structure.}\haizhou{briefly discuss the difference between unsupervised graph OOD and why exploring them is important.} In this study, we aim to investigate the robustness of graph self-supervised methods under different distribution shifts, shedding light on their performance in challenging graph OOD scenarios.
% Self-supervised methods seem to be more robust because the pre-training task is task-irerel and it hope to extract generic knowledges, eg,  contrastive methods xxx. In computer vision domain,  \cite{shi2022robust} found contrastive learning methods are more robust compared to supervised methods. But in the graph domain, it is xxx.
% Recent endeavors (Scarselli et al., 2018; Garg et al., 2020; Verma & Zhang, 2019) derive generalization error bounds for GNNs, yet they focus on in- distribution generalization and put little emphasis on distribution shifts, which are the main focus of our work. Furthermore, some up-to-date works explore GNN’s extrapolation ability for OOD data, e.g. unseen features/structures (Xu et al., 2021) and varying graph sizes (Yehudai et al., 2021; Bevilacqua et al., 2021). However, they mostly concentrate on graph-level tasks rather than node-level ones (see detailed comparison below). Moreover, some recent works probe into extrapolating features’ embeddings (Wu et al., 2021a) or user representations (Wu et al., 2021b) for open-world learning in tabular data or real systems for recommendation and advertisement. These works consider distribution shifts stemming from augmented input space or unseen entities, and the proposed models leverage GNNs as an explicit model that extrapolates to compute representations for new entities based on existing ones. In contrast, our work studies (implicit) distribution shifts behind observed data, and the proposed approach resorts to an implicit mechanism through the lens of invariance principle.
